Diffence: Fencing Membership Privacy With Diffusion Models

Deep learning models, while achieving remarkable performances, are vulnerable to membership inference attacks (MIAs). Although various defenses have been proposed, there is still substantial room for improvement in the privacy-utility trade-off. In this work, we introduce a novel defense framework against MIAs by leveraging generative models. The key intuition of our defense is to remove the differences between member and non-member inputs, which is exploited by MIAs, by re-generating input samples before feeding them to the target model. Therefore, our defense, called DIFFENCE, works pre inference, which is unlike prior defenses that are either training-time or post-inference time. A unique feature of DIFFENCE is that it works on input samples only, without modifying the training or inference phase of the target model. Therefore, it can be cascaded with other defense mechanisms as we demonstrate through experiments. DIFFENCE is designed to preserve the model's prediction labels for each sample, thereby not affecting accuracy. Furthermore, we have empirically demonstrated it does not reduce the usefulness of confidence vectors. Through extensive experimentation, we show that DIFFENCE can serve as a robust plug-n-play defense mechanism, enhancing membership privacy without compromising model utility. For instance, DIFFENCE reduces MIA accuracy against an undefended model by 15.8\% and attack AUC by 14.0\% on average across three datasets, all without impacting model utility. By integrating DIFFENCE with prior defenses, we can achieve new state-of-the-art performances in the privacy-utility trade-off. For example, when combined with the state-of-the-art SELENA defense it reduces attack accuracy by 9.3\%, and attack AUC by 10.0\%. DIFFENCE achieves this by imposing a negligible computation overhead, adding only 57ms to the inference time per sample processed on average.

==> sections/artifact.tex <==
% Artifact Appendix template for the NDSS Artifact Evaluation
% version 1.0 (20230620)

% remove the following block when merging the appendix with the camera-ready full paper
%%%

\section{Artifact Appendix}

% The artifact appendix is meant to be a self-contained document presenting a roadmap for setting up and evaluating your artifact. It should provide the following elements:
% \begin{enumerate}
% \item a list of the hardware, software, and configuration \textbf{requirements} for running the artifact;
% \item a clear description of how, and in what respects, the artifact \textbf{supports} the research presented in the paper;
% \item a guide for how others can \textbf{execute and validate} the artifact for its functional and usability aspects;
% \item the \textbf{major claims} made by your paper and a clear description of how to obtain data for each claim through your supplied artifact.
% \end{enumerate}

% Points 3-4 are not required if only the \textit{Available} badge is requested. Linking the paper claims to the artifact is a necessary step that allows artifact evaluators to functionally test and reproduce your results. Towards that end, explicitly list down items (e.g., results, plots, tables) from the paper and cross-reference them with the experiments to be reproduced.
 
% Unless otherwise stated, filling every section below with the requested contents is mandatory for participating in the artifact evaluation process. Section titles cannot be changed.

\subsection{Description \& Requirements}

% This section should list all the information necessary to recreate the experimental setup you used to run your artifact.

% Provide also a link to an archival repository where all the artifact's main components (software, datasets, documentation, etc.) can be accessed and, where this applies, the minimal hardware and software requirements to run your artifact.

% It is also very good practice to list and describe in this section benchmarks where those are part of your artifacts or simply have been used to produce results with it.

% \subsubsection{How to access}
% Describe here how to access your artifact. During the artifact evaluation, in case of a private repository, you should provide instructions on how to access it. For the camera-ready version of the appendix, you must provide a DOI link to the AEC-approved artifact version that you must upload by then to permanent storage.

% \subsubsection{Hardware dependencies}
% Simply write ``None." where this does not apply to your artifact.

% \subsubsection{Software dependencies} 
% Simply write ``None." where this does not apply to your artifact.

% \subsubsection{Benchmarks} 
% Describe here any data (e.g., datasets, models, workloads, etc.) required by the experiments with this artifact reported in your paper. Simply write ``None." where this does not apply to your artifact.


\subsubsection{How to Access}
The artifact is archived on Zenodo: \url{https://doi.org/10.5281/zenodo.13706131}. The corresponding GitHub repository can be found \url{https://github.com/SPIN-UMass/Diffence}.


\subsubsection{Hardware Dependencies}

The primary hardware dependencies are commodity GPUs, such as the NVIDIA Quadro RTX 8000 and NVIDIA GeForce RTX 2080 Ti, which were used in our experiments. Our code is designed to run on a university cluster, and we have modified the scripts to also work with standard commodity GPUs.

\subsubsection{Software Dependencies}

The main software dependencies include PyTorch, torchvision, TensorFlow, pandas, Opacus, scikit-learn, numpy, scipy, and matplotlib. We provide a conda environment file, \texttt{environment.yaml}, which can be used to install all necessary software dependencies with a single command using conda. Please refer to the README file for installation instructions.

\subsubsection{Benchmarks}

Benchmark datasets: CIFAR-10, CIFAR-100, and SVHN.
Models: Undefended models and models protected by different defense methods including SELENA, AdvReg, HAMP, RelaxLoss, DPSGD, and MemGuard. Additionally, models with \name (our method) deployed on top of the previously mentioned models.

We provide the aforementioned datasets and pretrained models, as well as the corresponding diffusion models used for \name.

\subsection{Artifact Installation \& Configuration}

First, download the artifact from the address provided in Section A.1, which includes the `environment.yaml` file. Run the following command to install the dependencies:

\begin{verbatim}
conda env create -f environment.yaml
\end{verbatim}

If you do not have conda installed, first install conda by following the instructions on their official documentation: \url{https://docs.conda.io/projects/conda/en/latest/user-guide/install/index.html}.



\subsection{Experiment Workflow}

The main workflow of the experiment includes:

1. Training target models:
   - This includes both undefended models and models with different defense techniques.

2. Testing models:
   - Measure test accuracy.
   - Evaluate membership privacy using different membership inference attacks (MIAs), assessed by metrics such as attack AUC and accuracy.

3. Deploying \name:
   - Apply \name to the above-tested models.
   - Re-evaluate model accuracy and the effectiveness of MIAs using the same methods.

4. Comparing results:
   - Compare the changes in model accuracy and membership privacy before and after deploying \name.


\subsection{Major Claims}

\begin{itemize}
\item (C1): \textsc{\name} can enhance the membership privacy of both undefended models and models with existing defenses without compromising their utility. This is proven by experiment (E1), with results mainly illustrated in Fig. 5 and additional references such as Table III.
\end{itemize}


\subsection{Evaluation}

\textsc{\name} can serve as a robust plug-and-play defense mechanism to enhance the membership privacy of both undefended models and models trained with state-of-the-art defenses without compromising model utility.

\textbf{Note:} Given the time constraints of the artifact evaluation, we recommend first evaluating the impact of \name on the undefended model and the SELENA model (the defense that achieves the best overall utility-privacy trade-off in our evaluation).

This evaluation demonstrates that \name enhances the defense against MIAs for both undefended models and the best-performing defense, without compromising accuracy. 
The results should be consistent with the conclusions in Fig. 5, showing that adding \name does not change model accuracy but reduces attack AUC and ACC to a comparable extent as described in Fig. 5.

Additionally, code and pre-trained models for other defense models are provided for anyone interested in conducting a comprehensive evaluation.

\subsubsection{Experiment (E1)}
\begin{figure*}
    \centering
    \includegraphics[width=1.0\linewidth]{New/sections/images_v1/artifact_utility.png}
    \caption{Example output showcasing the model accuracy from the evaluation files}
    \label{fig:artifact-utility}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=1.0\linewidth]{New/sections/images_v1/artifact_mia.png}
    \caption{Example output showcasing the recorded effectiveness of MIAs against the model}
    \label{fig:artifact-privacy}
\end{figure*}

This experiment verifies the model's accuracy and the effectiveness of MIAs before and after deploying \name.

\textit{[Preparation]}

\begin{enumerate}
  \item First, navigate to the folder of the dataset to be tested, e.g., CIFAR-10:
  \begin{quote}
  \texttt{cd cifar10}
  \end{quote}

  \item Download and partition the dataset:
  \begin{quote}
  \texttt{python data\_partition.py}
  \end{quote}

  \item Obtain the diffusion model used for \name:
  
  We provide our pretrained diffusion model checkpoints and instructions on how to download them in the repository.

(Optional) Train the diffusion model from scratch by following the instructions in the README file.

\end{enumerate}

\textit{[Execution]}

\begin{enumerate}
  \item Train the undefended model and models with existing defenses:

  We provide our pretrained models. You can find the download address in the repository.
  
  (Optional) You can retrain specific defended models using the commands listed in \texttt{all-train-all.sh}.

  \item Test model accuracy and membership privacy:
  \begin{quote}
  \texttt{cd evaluate\_MIAs}  \# Navigate to the test script folder \\
  \texttt{bash evaluate\_mia.sh --defense <defense name>}  \# defense name in \{undefended, selena, advreg, hamp, relaxloss, dpsgd\}
  \end{quote}
\end{enumerate}

After completion, the results of the above experiments will be saved in the \texttt{./results} folder.

\textit{[Results]}


The above process will save the corresponding results in \texttt{\name/<dataset\_name>/evaluate\_MIAs/results}. For example, file names such as \texttt{selena} and \texttt{selena\_w\_\name} correspond to the results of using SELENA defense alone and deploying \name on top of it, respectively. Each file records the model's accuracy (e.g., as shown in Fig. \ref{fig:artifact-utility}) and the effectiveness of MIAs against the model (as shown in Fig. \ref{fig:artifact-privacy}). The best attack ACC and AUC are used to indicate the level of the model's membership privacy.

The key results should be validated by comparing the changes in model accuracy and membership privacy.

% remove the following block when merging the appendix with the camera-ready full paper
%%%

\end{document}
%%%
